Multi-fidelity Reinforcement Learning Control for Complex Dynamical Systems

Controlling instabilities in complex dynamical systems is challenging in scientific and engineering applications. Deep reinforcement learning (DRL) has seen promising results for applications in different scientific applications. The many-query nature of control tasks requires multiple interactions with real environments of the underlying physics. However, it is usually sparse to collect from the experiments or expensive to simulate for complex dynamics. Alternatively, controlling surrogate modeling could mitigate the computational cost issue. However, a fast and accurate learning-based model by offline training makes it very hard to get accurate pointwise dynamics when the dynamics are chaotic. To bridge this gap, the current work proposes a multi-fidelity reinforcement learning (MFRL) framework that leverages differentiable hybrid models for control tasks, where a physics-based hybrid model is corrected by limited high-fidelity data. We also proposed a spectrum-based reward function for RL learning. The effect of the proposed framework is demonstrated on two complex dynamics in physics. The statistics of the MFRL control result match that computed from many-query evaluations of the high-fidelity environments and outperform other SOTA baselines.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%



% \section{Default Notation}

% In an attempt to encourage standardized notation, we have included the
% notation file from the textbook, \textit{Deep Learning}
% \cite{goodfellow2016deep} available at
% \url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
% is not required and can be disabled by commenting out
% \texttt{math\_commands.tex}.


% \centerline{\bf Numbers and Arrays}
% \bgroup
% \def\arraystretch{1.5}
% \begin{tabular}{p{1in}p{3.25in}}
% $\displaystyle a$ & A scalar (integer or real)\\
% $\displaystyle \va$ & A vector\\
% $\displaystyle \mA$ & A matrix\\
% $\displaystyle \tA$ & A tensor\\
% $\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
% $\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
% $\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
% $\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
% $\displaystyle \ra$ & A scalar random variable\\
% $\displaystyle \rva$ & A vector-valued random variable\\
% $\displaystyle \rmA$ & A matrix-valued random variable\\
% \end{tabular}
% \egroup
% \vspace{0.25cm}

% \centerline{\bf Sets and Graphs}
% \bgroup
% \def\arraystretch{1.5}

% \begin{tabular}{p{1.25in}p{3.25in}}
% $\displaystyle \sA$ & A set\\
% $\displaystyle \R$ & The set of real numbers \\
% $\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
% $\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
% $\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
% $\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
% $\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
% $\displaystyle \gG$ & A graph\\
% $\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
% \end{tabular}
% \vspace{0.25cm}




% \centerline{\bf Indexing}
% \bgroup
% \def\arraystretch{1.5}

% \begin{tabular}{p{1.25in}p{3.25in}}
% $\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
% $\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
% $\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
% $\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
% $\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
% $\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
% $\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
% $\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
% \end{tabular}
% \egroup
% \vspace{0.25cm}


% \centerline{\bf Calculus}
% \bgroup
% \def\arraystretch{1.5}
% \begin{tabular}{p{1.25in}p{3.25in}}
% % NOTE: the [2ex] on the next line adds extra height to that row of the table.
% % Without that command, the fraction on the first line is too tall and collides
% % with the fraction on the second line.
% $\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
% $\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
% $\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
% $\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
% $\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
% $\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
% $\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
% $\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
% $\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
% \end{tabular}
% \egroup
% \vspace{0.25cm}

% \centerline{\bf Probability and Information Theory}
% \bgroup
% \def\arraystretch{1.5}
% \begin{tabular}{p{1.25in}p{3.25in}}
% $\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
% $\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
% a variable whose type has not been specified\\
% $\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
% $\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
% $\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
% $\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
% $\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
% $\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
% $\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
% over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
% \end{tabular}
% \egroup
% \vspace{0.25cm}

% \centerline{\bf Functions}
% \bgroup
% \def\arraystretch{1.5}
% \begin{tabular}{p{1.25in}p{3.25in}}
% $\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
% $\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
%   $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
%   (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
% $\displaystyle \log x$ & Natural logarithm of $x$ \\
% $\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
% $\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
% $\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
% $\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
% $\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
% $\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
% \end{tabular}
%\egroup
%\vspace{0.25cm}

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}} 


\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}} 


\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> preamble.macros.tex <==

% Required packages
\usepackage{bm} % required for: \bm{}
\usepackage{amsfonts} % required for: \mathbb{}, \mathcal{}, ...

% Basic math commands
\newcommand{\func}[3]{\ensuremath{#1 : #2 \rightarrow #3}}
\newcommand{\spanV}{\ensuremath{\mathrm{span\hspace{0.05cm}}}}
\newcommand{\norm}[1]{\ensuremath{\left\| #1 \right\|}}

% Unconstrained optimization
\newcommand{\optunc}[2]{\underset{#1}{\text{minimize}} ~~ #2}

% Constrained optimization, 1 constraint
\newcommand{\optconOne}[3]{
\begin{aligned}
& \underset{#1}{\text{minimize}}
& & #2 \\
& \text{subject to} & & #3
\end{aligned}}

% Constrained optimization, 2 constraints
\newcommand{\optconTwo}[4]{
\begin{aligned}
& \underset{#1}{\text{minimize}}
& & #2 \\
& \text{subject to} & & #3 \\
& & & #4
\end{aligned}
}

% Constrained optimization, 3 constraints
\newcommand{\optconThree}[5]{
\begin{aligned}
& \underset{#1}{\text{minimize}}
& & #2 \\
& \text{subject to} & & #3 \\
& & & #4 \\
& & & #5
\end{aligned}
}

% Unconstrained optimization
\newcommand{\argoptunc}[2]{\underset{#1}{\arg\min} ~~ #2}

% First partial derivative
\newcommand{\pder}[2]{\ensuremath{\frac{\partial #1}{\partial #2}}}

% Second partial derivative
\newcommand{\pderTwo}[3]{\ensuremath{\frac{\partial^2 #1}{\partial #2 \partial #3}}}

% Third partial derivative
\newcommand{\pderThree}[4]{\ensuremath{\frac{\partial^3 #1}{\partial #2 \partial #3 \partial #4}}} %3rd partial derivative

\newcommand{\pderH}[3]{\ensuremath{\frac{\partial^{#3} #1}{\partial #2^{#3}}}}

% Total derviative
\newcommand{\oder}[2]{\ensuremath{\frac{d#1}{d#2}}}
% \newcommand{\oder}[2]{\ensuremath{D_{#2} #1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% FONTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Caligraphy
\newcommand{\Acal}{\ensuremath{\mathcal{A}}}
\newcommand{\Bcal}{\ensuremath{\mathcal{B}}}
\newcommand{\Ccal}{\ensuremath{\mathcal{C}}}
\newcommand{\Dcal}{\ensuremath{\mathcal{D}}}
\newcommand{\Ecal}{\ensuremath{\mathcal{E}}}
\newcommand{\Fcal}{\ensuremath{\mathcal{F}}}
\newcommand{\Gcal}{\ensuremath{\mathcal{G}}}
\newcommand{\Hcal}{\ensuremath{\mathcal{H}}}
\newcommand{\Ical}{\ensuremath{\mathcal{I}}}
\newcommand{\Jcal}{\ensuremath{\mathcal{J}}}
\newcommand{\Kcal}{\ensuremath{\mathcal{K}}}
\newcommand{\Lcal}{\ensuremath{\mathcal{L}}}
\newcommand{\Mcal}{\ensuremath{\mathcal{M}}}
\newcommand{\Ncal}{\ensuremath{\mathcal{N}}}
\newcommand{\Ocal}{\ensuremath{\mathcal{O}}}
\newcommand{\Pcal}{\ensuremath{\mathcal{P}}}
\newcommand{\Qcal}{\ensuremath{\mathcal{Q}}}
\newcommand{\Rcal}{\ensuremath{\mathcal{R}}}
\newcommand{\Scal}{\ensuremath{\mathcal{S}}}
\newcommand{\Tcal}{\ensuremath{\mathcal{T}}}
\newcommand{\Ucal}{\ensuremath{\mathcal{U}}}
\newcommand{\Vcal}{\ensuremath{\mathcal{V}}}
\newcommand{\Wcal}{\ensuremath{\mathcal{W}}}
\newcommand{\Xcal}{\ensuremath{\mathcal{X}}}
\newcommand{\Ycal}{\ensuremath{\mathcal{Y}}}
\newcommand{\Zcal}{\ensuremath{\mathcal{Z}}}

% Bold caligraphy
\newcommand{\Aboldcal}{\ensuremath{\boldsymbol{\mathcal{A}}}}
\newcommand{\Bboldcal}{\ensuremath{\boldsymbol{\mathcal{B}}}}
\newcommand{\Cboldcal}{\ensuremath{\boldsymbol{\mathcal{C}}}}
\newcommand{\Dboldcal}{\ensuremath{\boldsymbol{\mathcal{D}}}}
\newcommand{\Eboldcal}{\ensuremath{\boldsymbol{\mathcal{E}}}}
\newcommand{\Fboldcal}{\ensuremath{\boldsymbol{\mathcal{F}}}}
\newcommand{\Gboldcal}{\ensuremath{\boldsymbol{\mathcal{G}}}}
\newcommand{\Hboldcal}{\ensuremath{\boldsymbol{\mathcal{H}}}}
\newcommand{\Iboldcal}{\ensuremath{\boldsymbol{\mathcal{I}}}}
\newcommand{\Jboldcal}{\ensuremath{\boldsymbol{\mathcal{J}}}}
\newcommand{\Kboldcal}{\ensuremath{\boldsymbol{\mathcal{K}}}}
\newcommand{\Lboldcal}{\ensuremath{\boldsymbol{\mathcal{L}}}}
\newcommand{\Mboldcal}{\ensuremath{\boldsymbol{\mathcal{M}}}}
\newcommand{\Nboldcal}{\ensuremath{\boldsymbol{\mathcal{N}}}}
\newcommand{\Oboldcal}{\ensuremath{\boldsymbol{\mathcal{O}}}}
\newcommand{\Pboldcal}{\ensuremath{\boldsymbol{\mathcal{P}}}}
\newcommand{\Qboldcal}{\ensuremath{\boldsymbol{\mathcal{Q}}}}
\newcommand{\Rboldcal}{\ensuremath{\boldsymbol{\mathcal{R}}}}
\newcommand{\Sboldcal}{\ensuremath{\boldsymbol{\mathcal{S}}}}
\newcommand{\Tboldcal}{\ensuremath{\boldsymbol{\mathcal{T}}}}
\newcommand{\Uboldcal}{\ensuremath{\boldsymbol{\mathcal{U}}}}
\newcommand{\Vboldcal}{\ensuremath{\boldsymbol{\mathcal{V}}}}
\newcommand{\Wboldcal}{\ensuremath{\boldsymbol{\mathcal{W}}}}
\newcommand{\Xboldcal}{\ensuremath{\boldsymbol{\mathcal{X}}}}
\newcommand{\Yboldcal}{\ensuremath{\boldsymbol{\mathcal{Y}}}}
\newcommand{\Zboldcal}{\ensuremath{\boldsymbol{\mathcal{Z}}}}

% Block bold
\newcommand{\fbb}{\ensuremath{\mathbb{f}}}
\newcommand{\rbb}{\ensuremath{\mathbb{r}}}
\newcommand{\ubb}{\ensuremath{\mathbb{u}}}
\newcommand{\ybb}{\ensuremath{\mathbb{y}}}
\newcommand{\Abb}{\ensuremath{\mathbb{A}}}
\newcommand{\Cbb}{\ensuremath{\mathbb{C}}}
\newcommand{\Ebb}{\ensuremath{\mathbb{E}}}
\newcommand{\Gbb}{\ensuremath{\mathbb{G}}}
\newcommand{\Mbb}{\ensuremath{\mathbb{M} }}
\newcommand{\Nbb}{\ensuremath{\mathbb{N} }}
\newcommand{\Qbb}{\ensuremath{\mathbb{Q} }}
\newcommand{\Rbb}{\ensuremath{\mathbb{R} }}
\newcommand{\Vbb}{\ensuremath{\mathbb{V} }}
\newcommand{\Zbb}{\ensuremath{\mathbb{Z} }}

% Bold, italic arabic (capital)
\newcommand\Abm{{\ensuremath{\bm{A}}}}
\newcommand\Bbm{{\ensuremath{\bm{B}}}}
\newcommand\Cbm{{\ensuremath{\bm{C}}}}
\newcommand\Dbm{{\ensuremath{\bm{D}}}}
\newcommand\Ebm{{\ensuremath{\bm{E}}}}
\newcommand\Fbm{{\ensuremath{\bm{F}}}}
\newcommand\Gbm{{\ensuremath{\bm{G}}}}
\newcommand\Hbm{{\ensuremath{\bm{H}}}}
\newcommand\Ibm{{\ensuremath{\bm{I}}}}
\newcommand\Jbm{{\ensuremath{\bm{J}}}}
\newcommand\Kbm{{\ensuremath{\bm{K}}}}
\newcommand\Lbm{{\ensuremath{\bm{L}}}}
\newcommand\Mbm{{\ensuremath{\bm{M}}}}
\newcommand\Nbm{{\ensuremath{\bm{N}}}}
\newcommand\Obm{{\ensuremath{\bm{O}}}}
\newcommand\Pbm{{\ensuremath{\bm{P}}}}
\newcommand\Qbm{{\ensuremath{\bm{Q}}}}
\newcommand\Rbm{{\ensuremath{\bm{R}}}}
\newcommand\Sbm{{\ensuremath{\bm{S}}}}
\newcommand\Tbm{{\ensuremath{\bm{T}}}}
\newcommand\Ubm{{\ensuremath{\bm{U}}}}
\newcommand\Vbm{{\ensuremath{\bm{V}}}}
\newcommand\Wbm{{\ensuremath{\bm{W}}}}
\newcommand\Xbm{{\ensuremath{\bm{X}}}}
\newcommand\Ybm{{\ensuremath{\bm{Y}}}}
\newcommand\Zbm{{\ensuremath{\bm{Z}}}}

% Bold, italic arabic (lower)
\newcommand\abm{{\ensuremath{\bm{a}}}}
\newcommand\bbm{{\ensuremath{\bm{b}}}}
\newcommand\cbm{{\ensuremath{\bm{c}}}}
\newcommand\dbm{{\ensuremath{\bm{d}}}}
\newcommand\ebm{{\ensuremath{\bm{e}}}}
\newcommand\fbm{{\ensuremath{\bm{f}}}}
\newcommand\gbm{{\ensuremath{\bm{g}}}}
\newcommand\hbm{{\ensuremath{\bm{h}}}}
\newcommand\ibm{{\ensuremath{\bm{i}}}}
\newcommand\jbm{{\ensuremath{\bm{j}}}}
\newcommand\kbm{{\ensuremath{\bm{k}}}}
\newcommand\lbm{{\ensuremath{\bm{l}}}}
\newcommand\mbm{{\ensuremath{\bm{m}}}}
\newcommand\nbm{{\ensuremath{\bm{n}}}}
\newcommand\pbm{{\ensuremath{\bm{p}}}}
\newcommand\qbm{{\ensuremath{\bm{q}}}}
\newcommand\rbm{{\ensuremath{\bm{r}}}}
\newcommand\sbm{{\ensuremath{\bm{s}}}}
\newcommand\tbm{{\ensuremath{\bm{t}}}}
\newcommand\ubm{{\ensuremath{\bm{u}}}}
\newcommand\vbm{{\ensuremath{\bm{v}}}}
\newcommand\wbm{{\ensuremath{\bm{w}}}}
\newcommand\xbm{{\ensuremath{\bm{x}}}}
\newcommand\ybm{{\ensuremath{\bm{y}}}}
\newcommand\zbm{{\ensuremath{\bm{z}}}}

% Bold arabic (capital)
\newcommand\Abold{\ensuremath{\mathbf{A}}}
\newcommand\Bbold{\ensuremath{\mathbf{B}}}
\newcommand\Cbold{\ensuremath{\mathbf{C}}}
\newcommand\Dbold{\ensuremath{\mathbf{D}}}
\newcommand\Ebold{\ensuremath{\mathbf{E}}}
\newcommand\Fbold{\ensuremath{\mathbf{F}}}
\newcommand\Gbold{\ensuremath{\mathbf{G}}}
\newcommand\Hbold{\ensuremath{\mathbf{H}}}
\newcommand\Ibold{\ensuremath{\mathbf{I}}}
\newcommand\Jbold{\ensuremath{\mathbf{J}}}
\newcommand\Kbold{\ensuremath{\mathbf{K}}}
\newcommand\Lbold{\ensuremath{\mathbf{L}}}
\newcommand\Mbold{\ensuremath{\mathbf{M}}}
\newcommand\Nbold{\ensuremath{\mathbf{N}}}
\newcommand\Obold{\ensuremath{\mathbf{O}}}
\newcommand\Pbold{\ensuremath{\mathbf{P}}}
\newcommand\Qbold{\ensuremath{\mathbf{Q}}}
\newcommand\Rbold{\ensuremath{\mathbf{R}}}
\newcommand\Sbold{\ensuremath{\mathbf{S}}}
\newcommand\Tbold{\ensuremath{\mathbf{T}}}
\newcommand\Ubold{\ensuremath{\mathbf{U}}}
\newcommand\Vbold{\ensuremath{\mathbf{V}}}
\newcommand\Wbold{\ensuremath{\mathbf{W}}}
\newcommand\Xbold{\ensuremath{\mathbf{X}}}
\newcommand\Ybold{\ensuremath{\mathbf{Y}}}
\newcommand\Zbold{\ensuremath{\mathbf{Z}}}

% Bold arabic (lower)
\newcommand\abold{\ensuremath{\mathbf{a}}}
\newcommand\bbold{\ensuremath{\mathbf{b}}}
\newcommand\cbold{\ensuremath{\mathbf{c}}}
\newcommand\dbold{\ensuremath{\mathbf{d}}}
\newcommand\ebold{\ensuremath{\mathbf{e}}}
\newcommand\fbold{\ensuremath{\mathbf{f}}}
\newcommand\gbold{\ensuremath{\mathbf{g}}}
\newcommand\hbold{\ensuremath{\mathbf{h}}}
\newcommand\ibold{\ensuremath{\mathbf{i}}}
\newcommand\jbold{\ensuremath{\mathbf{j}}}
\newcommand\kbold{\ensuremath{\mathbf{k}}}
\newcommand\mbold{\ensuremath{\mathbf{m}}}
\newcommand\nbold{\ensuremath{\mathbf{n}}}
\newcommand\pbold{\ensuremath{\mathbf{p}}}
\newcommand\qbold{\ensuremath{\mathbf{q}}}
\newcommand\rbold{\ensuremath{\mathbf{r}}}
\newcommand\sbold{\ensuremath{\mathbf{s}}}
\newcommand\tbold{\ensuremath{\mathbf{t}}}
\newcommand\ubold{\ensuremath{\mathbf{u}}}
\newcommand\vbold{\ensuremath{\mathbf{v}}}
\newcommand\wbold{\ensuremath{\mathbf{w}}}
\newcommand\xbold{\ensuremath{\mathbf{x}}}
\newcommand\ybold{\ensuremath{\mathbf{y}}}
\newcommand\zbold{\ensuremath{\mathbf{z}}}

% Vector arabic (capital)
\newcommand\Avec{\ensuremath{\vec{A}}}
\newcommand\Bvec{\ensuremath{\vec{B}}}
\newcommand\Cvec{\ensuremath{\vec{C}}}
\newcommand\Dvec{\ensuremath{\vec{D}}}
\newcommand\Evec{\ensuremath{\vec{E}}}
\newcommand\Fvec{\ensuremath{\vec{F}}}
\newcommand\Gvec{\ensuremath{\vec{G}}}
\newcommand\Hvec{\ensuremath{\vec{H}}}
\newcommand\Ivec{\ensuremath{\vec{I}}}
\newcommand\Jvec{\ensuremath{\vec{J}}}
\newcommand\Kvec{\ensuremath{\vec{K}}}
\newcommand\Lvec{\ensuremath{\vec{L}}}
\newcommand\Mvec{\ensuremath{\vec{M}}}
\newcommand\Nvec{\ensuremath{\vec{N}}}
\newcommand\Ovec{\ensuremath{\vec{O}}}
\newcommand\Pvec{\ensuremath{\vec{P}}}
\newcommand\Qvec{\ensuremath{\vec{Q}}}
\newcommand\Rvec{\ensuremath{\vec{R}}}
\newcommand\Svec{\ensuremath{\vec{S}}}
\newcommand\Tvec{\ensuremath{\vec{T}}}
\newcommand\Uvec{\ensuremath{\vec{U}}}
\newcommand\Vvec{\ensuremath{\vec{V}}}
\newcommand\Wvec{\ensuremath{\vec{W}}}
\newcommand\Xvec{\ensuremath{\vec{X}}}
\newcommand\Yvec{\ensuremath{\vec{Y}}}
\newcommand\Zvec{\ensuremath{\vec{Z}}}

% Vector arabic (lower)
\newcommand\avec{\ensuremath{\vec{a}}}
\newcommand\bvec{\ensuremath{\vec{b}}}
\newcommand\cvec{\ensuremath{\vec{c}}}
\newcommand\dvec{\ensuremath{\vec{d}}}
\newcommand\evec{\ensuremath{\vec{e}}}
\newcommand\fvec{\ensuremath{\vec{f}}}
\newcommand\gvec{\ensuremath{\vec{g}}}
\newcommand\hvec{\ensuremath{\vec{h}}}
\newcommand\ivec{\ensuremath{\vec{i}}}
\newcommand\jvec{\ensuremath{\vec{j}}}
\newcommand\kvec{\ensuremath{\vec{k}}}
\newcommand\mvec{\ensuremath{\vec{m}}}
\newcommand\nvec{\ensuremath{\vec{n}}}
\newcommand\pvec{\ensuremath{\vec{p}}}
\newcommand\qvec{\ensuremath{\vec{q}}}
\newcommand\rvec{\ensuremath{\vec{r}}}
\newcommand\svec{\ensuremath{\vec{s}}}
\newcommand\tvec{\ensuremath{\vec{t}}}
\newcommand\uvec{\ensuremath{\vec{u}}}
\newcommand\vvec{\ensuremath{\vec{v}}}
\newcommand\wvec{\ensuremath{\vec{w}}}
\newcommand\xvec{\ensuremath{\vec{x}}}
\newcommand\yvec{\ensuremath{\vec{y}}}
\newcommand\zvec{\ensuremath{\vec{z}}}

% Bold greek (lower)
\newcommand\alphabold{{\ensuremath{\boldsymbol{\alpha}}}}
\newcommand\chibold{{\ensuremath{\boldsymbol{\chi}}}}
\newcommand\lambdabold{{\ensuremath{\boldsymbol{\lambda}}}}
\newcommand\betabold{{\ensuremath{\boldsymbol{\beta}}}}
\newcommand\etabold{{\ensuremath{\boldsymbol{\eta}}}}
\newcommand\gammabold{{\ensuremath{\boldsymbol{\gamma}}}}
\newcommand\deltabold{{\ensuremath{\boldsymbol{\delta}}}}
\newcommand\mubold{{\ensuremath{\boldsymbol{\mu}}}}
\newcommand\kappabold{{\ensuremath{\boldsymbol{\kappa}}}}
\newcommand\iotabold{{\ensuremath{\boldsymbol{\iota}}}}
\newcommand\rhobold{{\ensuremath{\boldsymbol{\rho}}}}
\newcommand\taubold{{\ensuremath{\boldsymbol{\tau}}}}
\newcommand\phibold{{\ensuremath{\boldsymbol{\phi}}}}
\newcommand\varphibold{{\ensuremath{\boldsymbol{\varphi}}}}
\newcommand\psibold{{\ensuremath{\boldsymbol{\psi}}}}
\newcommand\nubold{{\ensuremath{\boldsymbol{\nu}}}}
\newcommand\omegabold{{\ensuremath{\boldsymbol{\omega}}}}
\newcommand\sigmabold{{\ensuremath{\boldsymbol{\sigma}}}}
\newcommand\upsilonbold{{\ensuremath{\boldsymbol{\upsilon}}}}
\newcommand\varthetabold{{\ensuremath{\boldsymbol{\vartheta}}}}
\newcommand\xibold{{\ensuremath{\boldsymbol{\xi}}}}
\newcommand\zetabold{{\ensuremath{\boldsymbol{\zeta}}}}
\newcommand\epsilonbold{{\ensuremath{\boldsymbol{\epsilon}}}}

% Bold greek (upper)
\newcommand\Phibold{{\ensuremath{\boldsymbol{\Phi}}}}
\newcommand\Pibold{{\ensuremath{\boldsymbol{\Pi}}}}
\newcommand\Sigmabold{{\ensuremath{\boldsymbol{\Sigma}}}}
\newcommand\Gammabold{{\ensuremath{\boldsymbol{\Gamma}}}}
\newcommand\Omegabold{{\ensuremath{\boldsymbol{\Omega}}}}
\newcommand\Thetabold{{\ensuremath{\boldsymbol{\Theta}}}}
\newcommand\Lambdabold{{\ensuremath{\boldsymbol{\Lambda}}}}
\newcommand\Psibold{{\ensuremath{\boldsymbol{\Psi}}}}
\newcommand\Xibold{{\ensuremath{\boldsymbol{\Xi}}}}
\newcommand\Upsilonbold{{\ensuremath{\mathbf{\Upsilon}}}}

% Bold numbers
\newcommand\zerobold{\ensuremath{\mathbf{0}}}
\newcommand\onebold{\ensuremath{\mathbf{1}}}
\newcommand\twobold{\ensuremath{\mathbf{2}}}
\newcommand\threebold{\ensuremath{\mathbf{3}}}
\newcommand\fourbold{\ensuremath{\mathbf{4}}}
\newcommand\fivebold{\ensuremath{\mathbf{5}}}
\newcommand\sixbold{\ensuremath{\mathbf{6}}}
\newcommand\sevenbold{\ensuremath{\mathbf{7}}}
\newcommand\eightbold{\ensuremath{\mathbf{8}}}
\newcommand\ninebold{\ensuremath{\mathbf{9}}}

==> preamble.tikz.tex <==
\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{pgfplotstable, booktabs} % filecontents
\pgfplotsset{compat=1.9}

\usetikzlibrary{pgfplots.groupplots}
\usepgfplotslibrary{fillbetween}
\usetikzlibrary{calc,fit,matrix,arrows,automata,positioning,shapes}
\usetikzlibrary{arrows.meta}

\pgfplotsset{select coords between index/.style 2 args={
    x filter/.code={
        \ifnum\coordindex<#1\def\pgfmathresult{}\fi
        \ifnum\coordindex>#2\def\pgfmathresult{}\fi
    }
}}

\tikzset{
 invisible/.style={opacity=0},
 visible on/.style={alt={#1{}{invisible}}},
 alt/.code args={<#1>#2#3}{%
   \alt<#1>{\pgfkeysalso{#2}}{\pgfkeysalso{#3}}
 },
}

% Annotation of triangle with slope
\newcommand{\logLogSlopeTriangle}[5]
{
 % #1. Relative offset in x direction.
 % #2. Width in x direction, so xA-xB.
 % #3. Relative offset in y direction.
 % #4. Slope d(y)/d(log10(x)).
 % #5. Plot options.

 \pgfplotsextra
 {
  \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
  \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
  \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
  \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

  % Calculate auxilliary quantities, in relative sense.
  \pgfmathsetmacro{\xArel}{#1}
  \pgfmathsetmacro{\yArel}{#3}
  \pgfmathsetmacro{\xBrel}{#1-#2}
  \pgfmathsetmacro{\yBrel}{\yArel}
  \pgfmathsetmacro{\xCrel}{\xArel}
  %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))}
  % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

  \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
  \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
  \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
  \pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
  \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

  % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
  \coordinate (A) at (rel axis cs:\xArel,\yArel);
  \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
  \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

  % Draw slope triangle.
  \draw[#5]   (A)-- node[pos=0.5,anchor=north,scale=0.8] {1}
              (B)--
              (C)-- node[pos=0.5,anchor=west,scale=0.8] {#4}
              cycle;
 }
}

